Characterizing Large Language Models as Rationalizers of Knowledge-intensive Tasks

Large language models (LLMs) are proficient at generating fluent text with minimal task-specific supervision. Yet, their ability to provide well-grounded rationalizations for knowledge-intensive tasks remains under-explored. Such tasks, like commonsense multiple-choice questions, require rationales based on world knowledge to support predictions and refute alternate options. We consider the task of generating knowledge-guided rationalization in natural language by using expert-written examples in a few-shot manner. Surprisingly, crowd-workers preferred knowledge-grounded rationales over crowdsourced rationalizations, citing their factuality, sufficiency, and comprehensive refutations. Although LLMs-generated rationales were preferable, further improvements in conciseness and novelty are required. In another study, we show how rationalization of incorrect model predictions erodes humans' trust in LLM-generated rationales. Motivated by these observations, we create a two-stage pipeline to review task predictions and eliminate potential incorrect decisions before rationalization, enabling trustworthy rationale generation.

==> tex/discussion.tex <==
\section{Discussion}
\label{sec:discussion}
In this section, we discuss limitations of our proposed approach, implications of our findings, and potential future research directions.

\subsection{LLM as Rationalizers: The Ugly}

\subsubsection{The Achilles' Heel: Hallucination}
While LLMs have been proficient in natural language understanding tasks, with specialization in text generation, their most well-known limitation is hallucination. While the impressive capabilities of these models stem from the abundance of world knowledge encoded therein, such encoding is lossy.
Therefore, generalization of such lossily encoded knowledge could lead to ``memory distortion'', \ie  hallucination. LLM-generated rationales may suffer from 
similar hallucinations. While grounding on external knowledge, adopted by our approach, offers promise~\cite{peng2023check, mallen-etal-2023-trust}, the problem may not be entirely alleviated. Even though crowdworkers in our studies positively rated the factuality and insightfulness of the generated rationales, additional scrutiny is required before deploying such rationalizers in mission critical tasks. Unfortunately, detecting hallucination is a challenging problem and is a nascent research area a few recent approaches including self-consistency via sampling generated text~\cite{manakul2023selfcheckgpt,elaraby2023halo} or comparing parts of the same generated text~\cite{mundler2023self}. Other approaches towards
reducing hallucinations including repairing reasoning chains in chain-of-thought-prompting~\cite{zhao2023verify} and verifying generated text using external reliable sources~\cite{mei2023foveate}. Similar approaches can be adopted while generating rationales.

%Benchmarks of closed-source LLMs such as GPT-4 are also not publicly available~\cite{gpt-4}. As proposed by, 


% \begin{itemize}
%     \item measuring knowledge groundedness. how do we measure how much came from KG. how do we make sure it's actually knowledge grounded and not the LLMs prior knowledge.
% \end{itemize}

\subsubsection{Credible Rationalization and Fairwashing}
Despite the strength of rationales in 
interpretably explaining a model's decisions, 
critiques, in general, have raised concerns about
a phenomena of XAI tools called \emph{fairwashing} which 
may mislead users
into trusting biased or incorrect models~\cite{alikhademi2021can}.
For example, our proposed credible rationalization framework promotes
intervening potentially incorrect predictions while 
recommending various options for communicating rationales in a trustworthy manner such as notifying human experts via escalations, providing a disclaimer when in doubt, and correcting the prediction on-the-fly and then re-rationalizing, among others. However, simply averting potential
faithful yet incorrect rationalization may result in \emph{fairwashing} --- 
end-users' trust on the model may increase
due to an illusion of a highly performant rationalizer~\cite{aivodji2019fairwashing}.
Such fairwashing may have catastrophic consequences
if employed in real-world applications such as 
in medical domain, hiring platforms, and credit agencies.
Alikhademi et al.~\cite{alikhademi2021can}
proposes a framework for evaluating explainable AI tools with 
respect to their capabilities for detecting and addressing issues of bias and fairness
as well as their capacity to communicate these results to their users
clearly. Therefore, future implementations of the credible 
rationale should adopt similar strategies to safeguard against
these issue. Another research direction can be to study and characterize the strengths and weakness of different credible rationalization strategies 
to inform design guidelines.

\subsection{LLM as Rationalizers: The Bad}
\subsubsection{Choice-supportive Bias}
The refutation complete rationales generated using our workflow
promotes choice-supportive bias~\cite{lind2017choice}. In cognitive
science, choice-supportive bias refers to the propensity towards 
retroactively promote a selected option positively while de-emphasizing 
other options. In subjective domains such as CSQA~\cite{csqa},
there may be multiple viable options depending on perspective.
As has been demonstrated in Section~\ref{sec:acc_fine}, crowdworkers
treated rationales of CSQA task less positively on aspects such refutation
convincingness. Future iterations of the rationalization
framework may address this issue. One approach can be to employ
self-consistency-based strategies~\cite{mei2023foveate, mundler2023self} to evaluate whether corroboration
of different choices are at odds with each other and 
repair rationales accordingly~\cite{zhao2023verify}.

\subsubsection{Scaling Responsibly}
While LLMs enable scaling up the rationalization process, as highlighted in the preceding sections, appropriate guardrails should be incorporated before any real-world adoption of such strategies. Besides the methodological and ethical concerns, an often overlooked aspect with the recent hype of LLMs has been \emph{Green AI}~\cite{schwartz2020green}. While the environmental impact and financial cost of pre-training of such large language models have been highlighted by existing work~\cite{10.1145/3442188.3445922}, employing LLMs to scale up downstream applications such as rationale generation can have similar effects. As open-source models continue to improve, closed-source and private LLMs such as GPT-3~\cite{brown2020language} remain more popular. Even in our proposed rationalizer one contributing factor in using GPT-3.5 as opposed to more advanced GPT-4 has been the generation cost. Moreover, when the ML deployment pipeline is considered as a whole, inference consumes the majority of compute resources, accounting for anything from between 70$\%$ to 90$\%$~\cite{weng2022mlaas,wu2022sustainable}. Knowledge distillation approaches can be adopted to avoid costly pre-training~\cite{wang2023scott} while materialization
of rationales to avoid repeating rationalizing the same task can be possible approaches to handle such issues.

\subsection{LLM as Rationalizers: The Good}

\subsubsection{Learning from Human Feedback}
Existing work on rationale generation~\cite{wiegreffe-etal-2022-reframing}  showcases the promise of fine-tuning a downstream classification model, on crowdworker feedback of rationales, to detect acceptable rationale. 
However, acceptability is coarse-grained metric and it is unclear which fine-grained aspect contributes to such acceptance in a given setting. 
In our studies, we collected crowdworker feedback on fine-grained rationale properties. These signals can be similarly employed to train models than characterize generated rationales along those access besides the coarse-grained acceptability and human preference metric. However, with the expansion of properties, large-scale studies with more crowdworkers may be required. Such an approach has similarities to reinforcement learning with human feedback~\cite{ouyang2022training} an increasingly popular mechanism where the goal is to align language models with user intent on a wide range of tasks by fine-tuning with human feedback. Similar strategy can be adopted to build models trained on rich human feedback collected in out studies along various characteristics of rationales.  


\subsubsection{Distilling Knowledge via Rationales}
As mentioned earlier, knowledge distillation strategies can help reduce carbon footprint by training a smaller model based on generations of demonstrations from a larger model. For example, SCOTT~\cite{wang2023scott} 
is a faithful knowledge distillation method that trains a small, self-consistent model using an LLM (teacher model that is orders of magnitude larger than the student.) The key focus of the work is on generating faithful rationales that can be used to train the student model and improve it's prediction task performance. Similar ideas can be adopted to train smaller knowledge-intensive task models for downstream tasks such as question answering. 
In this setting, the LLM plays the role of an artificial crowdworker
generating training examples for a downstream model.
Similar to data quality issues with human crowdworkers~\cite{douglas2023data}, the generated rationales may exhibit limitations such as hallucination and choice supportive bias, which practitioners should be mindful of. 

\subsection{Study Limitations}

There are a few limitations of the various human subject studies we conducted.
First, as we conducted the crowdsourced study on Amazon Mechanical Turk, our findings may not generalize to other platforms and feedback provided in in-person lab-based studies. Second, none of the human subject studies involved follow-up interviews and therefore, lack any qualitative insights. Such a setting also prevented us from gaining additional insights into the thought process of the participants. However, conducting such large-scale studies in an in-person setup introduces time and logistics constraints. Second, the final human subject study was a confirmatory study instrumenting designs of existing studies in the context of rationalization. In future, a more involved lab-based or a large-scale crowdsourced study could be conducted to make stronger claims about the observations. Finally, besides the study-specific limitations, all of the experiment observations were obtained in the context of GPT-3.5 \code{text davinci 003} and may not generalize all LLMs, both closed- and open-source.
